Facial Action Unit Detection and Intensity Estimation from Self-supervised Representation

As a fine-grained and local expression behavior measurement, facial action unit (FAU) analysis (e.g., detection and intensity estimation) has been documented for its time-consuming, labor-intensive, and error-prone annotation. Thus a long-standing challenge of FAU analysis arises from the data scarcity of manual annotations, limiting the generalization ability of trained models to a large extent. Amounts of previous works have made efforts to alleviate this issue via semi/weakly supervised methods and extra auxiliary information. However, these methods still require domain knowledge and have not yet avoided the high dependency on data annotation. This paper introduces a robust facial representation model MAE-Face for AU analysis. Using masked autoencoding as the self-supervised pre-training approach, MAE-Face first learns a high-capacity model from a feasible collection of face images without additional data annotations. Then after being fine-tuned on AU datasets, MAE-Face exhibits convincing performance for both AU detection and AU intensity estimation, achieving a new state-of-the-art on nearly all the evaluation results. Further investigation shows that MAE-Face achieves decent performance even when fine-tuned on only 1\% of the AU training set, strongly proving its robustness and generalization performance.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> zzz.backup/method_ard_bak.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Method}
\subsection{Problem Definition}
% 1.binary classfication
% 2.current challenges(lack data[cite somw works] overfitting[class imbalance, id, training/test data, illumination ])
% 3.large-scale pretraining , benefits
% 4.our method
As mentioned above, this work addresses both problems of AU detection and intensity estimation. Specifically, the AU detection aims to recognize occurrence or absence of AUs in an facial image. Since there exists multiple AUs in an input image, the AU detection is a multi-label classification problem. It aims to perform the AU binary classification (i.e. 0 for absence and 1 for presence) for n AUs: $P=[p_1,...,p_i,...,p_n]$, where $i \in {0,1}$ and $n$ is the total number of targeting AUs in the used dataset. Moreover, the AU intensity estimation are defined as six discrete levels from 0 to 5 that indicates various degrees of facial action movements, where 0 and 5 indicate the lowest and the highest activation degree, respectively. The target of AU intensity estimation task is to regress the AU intensity levels for n AUs, which is termed as $L=[l_1,...,l_i,...,l_n]$, where $i \in {0,1,...,5}$. 

It has been mentioned that the AU detection or intensity estimation suffer from the overfitting to the training data due to limited amount of available data in the released datasets (Please refer to Section \ref{}) \cite{}. Furthermore, our work attempts to recognize the mentioned overfitting as three aspects, including the overfitting to AU labels, the overfitting to identities, the overfitting to attributes, which will be detailed as follows.

\begin{itemize}
\item \textbf{Overfitting to AU labels.} It is well known that Data imbalance is a common issue for image recognition\cite{chou2020remix}\cite{liu2019large}\cite{cui2019class}, which may bias neural networks to the majority classes when the training data is heavily imbalanced. Similarly, AU related tasks also suffer from this problem due to the label distribution imbalance existed in AU datasets. Specifically, it can be summarized as AU class and AU combination distribution imbalance.  Firstly, as shown in column (a) and (b) of Figure \ref{fig:BP4D_data_distribution},\ref{fig:BP4D+_data_distribution} and \ref{fig:DISFA_data_distribution}, there are severe class distribution imbalance for all three AU datasets(Please refer to Secontion \ref{section:experiments_datasets}). In BP4D and BP4D+, samples of AU6, AU7, AU10, AU12 and AU14 are observably far more than other AUs, while AU4, AU12 and AU25 are the dominant classes in DISFA. In fact, as shown in Figure \ref{fig:dataset_network_performance}, it can be observed  that the detection performance of previous works(Please refer to Tab \ref{table:results:au_det_bp4d},\ref{table:results:au_det_bp4d+} and \ref{table:results:au_det_disfa}) for each AU is consistent with the AU class distribution. For example, in BP4D dataset, the accuracy of most networks on majority classes like AU6, AU7, AU10, AU12 are much better than that on minority classes of AU1,AU2,AU4,AU15,AU23 and AU24. This shows that previous works based on deep learning training tends to overfit to the dominant AU classes. % \textcolor{red}{How about making a figure to show the quantity of AU labels or their distribution.} As shown in Figure \ref{}, .... imbalance. .... tends to AUx and AUx. In fact, observing the results from previous works, the detection and estimation performance is consistent with the data distributions. Furthermore, AU combination......
% It means that the performance of deep models are critically influenced by the AU label distribution of training datasets. The annotation of AUs needs strong domain expertise and is time-consuming\cite{niu2019multi}\cite{yang2021exploiting}, thus existing data-driven methods are unable to avoid the dilemma of lacking sufficient AU label data and tends to overfit on the AU label. Firstly, the AU classes distributions vary between training and testing set(i.e. some AUs may occur only in training set), which results in the AU class overfitting.
% due to that AUs occur with facial expression and the occurrence of each expression class varies in frequency, there are severe class imbalance in available AU datasets and class distribution diversity between training and testing data set (i.e. some AUs may occur only in training set).
\begin{figure*}[!t]
    \centering
    \includegraphics[ width=18cm]{images/dataset_network_performance.pdf}
    %\vspace{-0.5em}
     \caption{The AU detection performance for several networks and the AU class samples distributions for BP4D, BP4D+ and DISFA, respectively, from which wee can see the networks' performances are consistent with the AU class distributions}
    \label{fig:dataset_network_performance}
\end{figure*}
%%%%%%%%%%%%%
Secondly, the AU combinations distribution is also imbalance for available AU datasets. Facial expressions can be realized by certain combination of different AUs. For instance, a happy expression might be the combination of AU6 and AU12, while a sad expression may involve AU1 and AU17. There are numerous AU relations of facial expressions in daily life. However, as shown in Figrue \ref{fig:BP4D_data_distribution},\ref{fig:BP4D+_data_distribution} and \ref{fig:DISFA_data_distribution}, there are only 102, 1669 and 1132 AU combinations in DISFA, BP4D and BP4D+, which are inadequate to cover all kinds of AU relationships. Moreover, the samples for most of the AU combinations are less than 50, while only 1\%, 2\% and 12\% AU combinations of BP4D, BP4D+ and DISFA have more than 1000 samples, in which the distribution of AU combinations follows a long-tailed distribution(As shown in column d of Figure \ref{fig:BP4D_data_distribution},\ref{fig:BP4D+_data_distribution} and \ref{fig:DISFA_data_distribution}). To sum up, the facts that available AU datasets are imbalanced in AU class and AU combination distribution may lead to overfitting to AU labels. 
% The bias of AU relation distribution in training and testing set may lead to AU relation overfitting. 

\item \textbf{Overfitting to identities}. A facial expression image can be separated to the identity cues and the motion cues related to emotion such as AUs\cite{xiang2017linear}, where the former ones are useless for facial action unit analysis. Thus it is expected to extract more AU related cues and disentangle with face identity in facial action unit related tasks. The identity cues include two aspects and we call them identity-specific expression appearance(ISA) and identity-specific expression custom(ISC). ISA reflects the individual differences in facial expression appearance like face shape, texture and skin color, etc\cite{chu2013selective}. ISC indicates the individual behavior customs of expressing emotions\cite{chen2022causal}. To be specific, when different persons express same expression, except for universal AU relations that are shared by all identities, there are some identity-specific AU combinations depended on the facial behavior custom of specific identity \cite{chen2022causal}\cite{LP}. In addition, the identities of available AU datasets(41,140 and 27 subjects in BP4D, BP4D+ and DISFA) are too few to cover all possible identity-specific AU relation varieties. All the above factors may make the deep learning model suffer from identity overfitting.

\item \textbf{Overfitting to attributes}. Some  other attributes irrelated to identity and expression like background and illumination  may also leads to overfitting.  Most AU datasets are captured in the lab, where the camera view is stable and the environment is changeless. The models trained merely on these datasets may be adaptive to dataset-specific attributes and less generic. However, the capture environments of testing data maybe in the wild, which vary a lot from the training data in background, illumination, view, pose, makeup, etc.  Thus the performance of models may decline seriously when applied to in-the-wild data. In short, previous works trained merely based on AU datasets tends to be data attributes overfitting\cite{niu2019multi}.


\end{itemize}

%Though some previous works have tried to tackle this problem with a auxiliary task like expression recognition by utilizing extra dataset, their  performance are still limited to the data scale because their supervised training strategy.
To alleviate above problems, we consider to construct a powerful and robust facial expression feature extractor which is trained on large-scale facial datasets without annotation in a self-supervised paradigm. Since the pretraining datasets are scrabbed from web and totally in the wild, they  contains numerous expression classes and relieve AU class and combination distribution imbalance problem. The numerous identies and various environment conditions, on the other hand, reduce the identity and environment overfitting risks. 

Our proposed method is simple yet effective, which contains two parts, namely a feature extractor based on pretrained MAE and a classifier head. In the following sections we will introduce each component in detail.

\subsection{Framework Overview}
As shown in Figure\ref{fig:pipeline}, our framework includes two stages, namely pretraining task stage(stage1) and AU related task stage(stage2). The framework of the pretraining stage is MAE, which contains a VIT encoder and a light decoder. The AU related task stage contains the same VIT encoder which pretrained from stage1 while it has a linear head to output the predicted AU results(occurrence probability or intensity value).

In the pretraining stage, the input facial data are randomly sampled from large scale facial datasets without AU anotations and the target is to train a strong and robust facial feature extractor. In the AU related task stage, We utilize the pretrained VIT encoder in stage1 as our feature extractor to extract powerful facial features. The input facial data are randomly sampled from AU datasets. Particularly, in this stage the facial data are not masked, in other word, all the pathches of input data are fed into the pretrained VIT encoder. We finetune the whole network to get the AU predicted results and update the whole network parameters.

\subsection{MAE Feature Extractor Pretraining}
Unlike other pretraining works for facial action unit which is ether directly on AU detection task or on related task like expression recognition with limited labeled data, our insight is to fully tap the potential of numerous facial data without annotation. Following MAE, we take advantage of the encoder-decoder structure as our pretraining framework. This section will introduce the details of our data processing and network pretraining.

% MAE Pretraining
\textbf{Pretraining with Masked Image Encoding.}
 We choose a simple yet efficient pretraining task, a self-supervised paradigm that partially masks the facial image patches and then reconstructs them. The encoder and decoder are denoted as $f(\cdot)$ and $d(\cdot)$. Given a facial image $I$, we first crop it into uniform non-overlapping patches $I = \{I_i\}_{n \times n}$, where n is the number of patches in the width or height direction, then we randomly sample them by a mask ratio $mr$ to get the masked patches $I^m = \{I_i\}^{mr}_{n \times n}$. The pretraining task can be denoted as:
\begin{equation}
\{I_i\}_{n \times n}= d(f(\{I_i\}^m_{n \times n})),
\end{equation}

This ensures us to obtain our strong and transferable feature extractor $f(\cdot)$.
A prominent option is the mask ratio $mr$. By masking out a large portion of the image
patches ($mr=75\%$), the MAE encoder is forced to extract high-level semantic information from the patches, where low-level features are not enough to predict the original image
contents.


\textbf{Pretraining Details.}
Following MAE[], we keep most of the pre-training setups the same, except:
\begin{itemize}
    \item [(1) ]
    We pre-train the model with facial image datasets, designed specifically for facial analysis tasks. 
    \item [(2) ]
     We use ViT-Base as the backbone in our experiments. As long as more computational resources are available, the results in this paper can be further improved with bigger backbone such as ViT-Large, ViT-Huge or ViT-Huge-448 variants. Rather than using bigger models, ViT-Base backbone shows the effectiveness of the method itself. More importantly, the ViT-Base model is more feasible for deploying.
    \item [(3) ]
    Since the face dataset is a subset of the general image dataset, instead of pre-training from scratch, we initialize the encoder weights from ImageNet-1k pre-trained MAE. This will boost the pre-training stage, requiring less epochs to converge. Note that it's also viable to pre-train from scratch as in the original MAE. In our early experiments, the AU model pre-trained from scratch still outperforms the previous bests.
    \item [(4) ]
    L1 loss is used as the loss function, replacing mean squared error (aka. L2 loss) proposed in the original MAE. As MAE directly reconstructs pixels, and L1 loss usually performs better than L2 loss in image restoration problems[], L1 loss is worth a try in MAE pre-training. In our experiments, L1 pre-trained MAE improves sharpness of the reconstructed images, and fine-tuned MAE also performs better with L1 pre-training.
\end{itemize}

\textbf{Pretraining Dataset \& Pre-processing.}
We build up our pre-training dataset from 4 datasets,designed for various facial tasks, These datasets are concatenated to form a large set. The size of the combined dataset is ~2.17M, with all the labels removed. 
\begin{enumlist}
\item AffectNet[], 960k, faces not aligned
\item CASIA-WebFace[], 494k, faces not aligned
\item IMDB-WIKI[], 514k, faces not aligned
\item CelebA[], 203k, faces aligned
\end{enumlist}

The proposed pre-training dataset is not very large. This benefits from the pre-training mechanism of MAE, where 75\% of the input image patches are masked out. The random masking can be viewed as strong data augmentation, which regularizes the training procedure and prevent overfitting even after 1600 epochs.

Nevertheless, we can still benefit from large-scale pre-training to further improve the performance. As labels are not required, it's quite easy to scale up the pre-training dataset from any dataset with face images. e.g. FaRL[] proposed to build up LAION-Face dataset by extracting face images from LAION-400M dataset[], which consists of ~50M facial image-text pairs.

The pre-training data are pre-processed as following:
\begin{enumlist}
\item We clean up the dataset by dropping corrupt files and images with too low resolution, e.g. either width or height is less than 64 (the threshold may change for each dataset).
\item RetinaFace[] is applied to detect faces and 5-point facial landmarks. Images with no face detected are dropped. Face images are aligned by rotating, bilinear interpolation is applied to suppress aliasing. The rotation angle is extracted from the coordinates of the two eyes in the facial landmarks.
\item RetinaFace is applied again to detect facial bounding box. A square region containing the bounding box is cropped to get the final face image.
\end{enumlist}

%\subsection{Transfer Learning on Action Units.}
\subsection{End-to-end fine-tuning on Action Units}
The pre-training task yields a powerful feature extractor, which can capture fine-grained facial features, served as an optimal network initialization. Thus in downstream tasks, we can train our AU detection network and AU intensity estimation network with limited labeled data. This section will introduce the implementation details for fine-tuning.

\textbf{Fine-tuning on Action Unit.}
In fine-tuning stage, all image patches are fed into the MAE encoder without masking. We extract features from the encoder output. The MAE decoder is dropped because there's no more need for reconstructing pixels. Then, global average pooling is applied to the features, followed by a LayerNorm[]. Finally, a fully connected layer is added to the end of the network, served as the classification head.

\textbf{Preprocessing for fine-tuning Datasets:} same as (ii) and (iii) in pre-training pre-processing, face detection, face alignment and face cropping is applied to extract aligned face images from the original datasets.

In common practices, face detection and face alignment plays an important role in facial recognition tasks. Therefore, it's natually to perform face alignment before feeding a face image to the AU model. We follow this practice in our fine-tuning stage, but a question raises in the pre-training stage.

By reconstructing pixels from natural images, the original MAE yields a generic image encoder, which can be easily adapted to various downstream vision tasks. What about MAE-Face? With aligned face images for both pre-training and fine-tuning, it is expected to be good in experimental cases, but may at the price of losing generality, e.g. lower precision when predicting non-aligned faces. With detailed experiments, We will explain this question in Section~\ref{section:ablation:data_preprocessing}.

\subsection{Loss Functions}
% AU Detection Fintuning
% AU Intensity Estimation Fintuning
Our pretraining procedure is a mask-then-predict task, which aims to predict the masked patches. The loss of pretraining task is $\mathcal{L}_{pre}$. We then validate our pretrained model on both AU detection and AU intensity estimation tasks, whose losses are denoted as $\mathcal{L}_{det}$ and $\mathcal{L}_{int}$, respectively, each of them is introduced in detail in the following.

\textbf{Loss of MAE pretraining.} Suppose there are $K$ masked patches in the input $I^m = \{I_i\}^{mr}_{n \times n}$. To predict the $K$ masked patches accurately, we utilize pixel-wise L1 loss to constrain the distance between the prediction ($\hat m_k$) and ground-truth ($m_k$) of the masked patches. Thus ${L}_{pre}$ can be denoted as:
\begin{equation}
\mathcal L_{pre} = \sum_{k=1}^{K} || m_k - \hat m_k ||,
\end{equation}

\textbf{Loss of AU detection.} To constrain the AU detection results to be as close as possible with AU ground-truth, we formulate it as a multi-label binary classification problem, where each AU label is a binary. Thus $\mathcal{L}_{det}$ is defined as:
\begin{equation}
\mathcal L_{det} = -\sum_{i=1}^{N} [p_i log \hat{p}_i + (1 - p_i) log(1-\hat{p}_i)],
\end{equation}
where $N$ is the number of AUs, $\hat p_i$  denotes the predicted probability which is the model output activated by a sigmoid function, and $p_i$ denotes the binary ground-truth of $AU_{i}$.

\textbf{Loss of AU intensity estimation.} Since the AU intensity values are annotated as discrete integers in 0$\sim$5, we normalize the ground-truth values to 0$\sim$1. Then, the goal of our model is to regress the normalized AU intensity values. We use L2 distance to minimize the distance between the predicted value $\hat v_i$ and ground-truth $v_i$ for $AU_{i}$, thus $\mathcal{L}_{int}$ is denoted as:
\begin{equation}
\mathcal L_{int} = \sum_{i=1}^{N} || v_i - \hat v_i ||^2_2,
\end{equation}
During inference, the model output is scaled to the original 0$\sim$5 range for evaluation.


==> zzz.backup/method_ard_bak_20221009.tex <==
% LaTeX Error: Can be used only in preamble.
% \usepackage{cleveref}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Method}

In this section we will introduce our proposed method in detail. Firstly we describle the problem definition of AU detection and intensity estimation, representing the overfitting problems commonly exist in previous works. Then, we give an overview of our proposed framework. After that, we introduce the pre-training and fine-tuning procedure. Finally, we present the training loss used in our works.


%%%%%%%%%%%%%%%%
\subsection{Problem Definition}
% 1.binary classfication
% 2.current challenges(lack data[cite somw works] overfitting[class imbalance, id, training/test data, illumination ])
% 3.large-scale pre-training , benefits
% 4.our method

As mentioned above, this work addresses both problems of AU detection and intensity estimation. Specifically, the AU detection aims to recognize occurrence or absence of AUs in an face image. Since there exists multiple AUs in an input image, the AU detection is a multi-label classification problem. It aims to perform the AU binary classification (i.e. 0 for absence and 1 for presence) for n AUs: $P=[p_1,...,p_i,...,p_n]$, where $p_i \in {0,1}$ and $n$ is the total number of AUs in the target dataset. Moreover, the AU intensity estimation are defined as six discrete levels from 0 to 5 that indicates various degrees of facial action movements, where 0 and 5 indicate the lowest and the highest activation degree, respectively. The target of AU intensity estimation task is to regress the AU intensity levels for n AUs, which is termed as $L=[l_1,...,l_i,...,l_n]$, where $l_i \in {0,1,...,5}$.

It has been mentioned that the AU detection or intensity estimation suffers from overfitting to the training set due to the limited amount of available data in the released datasets (please refer to Section~\ref{})\cite{}. Furthermore, our work attempts to recognize the mentioned overfitting as three aspects, including the overfitting to AU labels, the overfitting to identities, the overfitting to attributes, which will be detailed as follows.

%\begin{widelist}
%\item
\textit{Overfitting to AU labels.} It is well known that data imbalance is a common issue for image recognition\cite{chou2020remix}\cite{liu2019large}\cite{cui2019class}, which may bias neural networks towards the majority classes when the training data is heavily imbalanced. Similarly, AU-related tasks also suffer from this problem due to the imbalance of label distribution existed in the available datasets. Specifically, the imbalance involves individual AU classes and AU combinations. \cref{fig:BP4D_data_distribution,fig:BP4D+_data_distribution,fig:DISFA_data_distribution} show the distributions of AU classes from three commonly-used datasets (please refer to Section~\ref{section:experiments_datasets} for more details). We can clearly observe the imbalance of the distributions of AU classes and AU combinations. For example, \cref{fig:BP4D_data_distribution,fig:BP4D+_data_distribution} show that samples of AU6,7,10,12,14 are observably far more than the other AUs in BP4D and BP4D+; \cref{fig:DISFA_data_distribution} shows that AU4,12 and AU25 are the dominant classes in DISFA. On the other hand, \cref{fig:dataset_network_performance} shows the AU detection performance of previous works (please refer to \cref{table:results:au_det_bp4d,table:results:au_det_bp4d+,table:results:au_det_disfa} for the results from more existing works.). It can be observed that the performance (please refer to \cref{table:results:au_det_bp4d,table:results:au_det_bp4d+,table:results:au_det_disfa}) is consistent with the AU class distributions in \cref{fig:BP4D_data_distribution,fig:BP4D+_data_distribution,fig:DISFA_data_distribution}. For example, in the BP4D dataset, the performance F1 of previous works on majority classes like AU6,7,10,12 tends to be much higher than that on minority classes of AU1,2,4,15,23,24. This shows that previous works suffer from overfitting to the dominant AU classes.
\begin{figure*}[!t]
    \centering
    \includegraphics[ width=18cm]{images/dataset_network_performance.pdf}
    %\vspace{-0.5em}
     \caption{The AU detection F1-score for several SOTA frameworks (SEV-Net\cite{yang2021exploiting},MHSA-FFN\cite{jacob2021facial},CIS-Net\cite{chen2022causal},CaFNet\cite{chen2021cafgraph},and MGRR-Net\cite{ge2022mgrr}) and the AU class samples distributions for BP4D, BP4D+ and DISFA, respectively, from which wee can see that the F1-score on each AU of all networks are consistent with the AU class distributions}
    \label{fig:dataset_network_performance}
\end{figure*}
%%%%%%%%%%%%%

Furthermore, \cref{fig:BP4D_data_distribution,fig:BP4D+_data_distribution,fig:DISFA_data_distribution} also show the AU combination distributions from three commonly-used datasets (please refer to Section~\ref{section:experiments_datasets} for more details). As observed, the AU combination distributions are also imbalance. \cref{fig:BP4D_data_distribution,fig:BP4D+_data_distribution,fig:DISFA_data_distribution} show the imbalanced distributions of AU combinations in DISFA, BP4D and BP4D+. The samples for most of the AU combinations are less than 50, while only 1\%, 2\% and 12\% AU combinations of BP4D, BP4D+ and DISFA have more than 1000 samples, so the distribution of AU combinations follows a long-tailed distribution (As shown in column d of Figure \cref{fig:BP4D_data_distribution,fig:BP4D+_data_distribution,fig:DISFA_data_distribution}). Additionally, we observe 102, 1669 and 1132 kinds of AU combinations in DISFA, BP4D and BP4D+, which are inadequate to cover all possible kinds of AU combinations. The long-tail and limited distribution cannot fully reflect AU relationships in natural facial expressions.

% The bias of AU relation distribution in training and testing set may lead to AU relation overfitting.
% To sum up, the imbalance in the distributions of AU class and AU combination probably lead to the overfitting to AU labels.
To sum up, due to the imbalanced distributions of AU class and AU combinations, it is very likely for a trained model to overfit to the AU labels.

%\item 
\textit{Overfitting to identities}. It is expected to move out identity information from the expression latent representations for the AU tasks. Unfortunately, some expressions are scare and only appear on a few specific identities, leading to entanglement of these expressions and identities. Moreover, this entanglement is also aggravated, as the identities of available AU datasets (41,140 and 27 subjects in BP4D, BP4D+ and DISFA) are too few. \textcolor{red}{Can we make a few examples to show this overfitting.}

%Thus it is expected to extract more AU-related cues and disentangle with face identity in facial action unit related tasks. Some AU combinations are scare and only appear on specific identities, seems to entangle with these identities. Besides, the identities of available AU datasets(41,140 and 27 subjects in BP4D, BP4D+ and DISFA) are too few to cover all possible identity-specific AU relation varieties. All the above factors may make the deep learning model suffer from identity overfitting.

%A facial expression image can be separated to the identity cues and the motion cues related to emotion such as AUs\cite{xiang2017linear}, where the former ones are useless for facial action unit analysis. 

%\item 
\textit{Overfitting to attributes}. Some other attributes unrelated to expression, like background, illumination, view, pose and makeup, are hard to leave out from the expression latent representations for the AU tasks, since their scarcity leads to their entanglement with specific expressions. \textcolor{red}{Can we make a few examples to show this overfitting.}

%also lead to overfitting. Most AU datasets are captured in the lab, where the camera view is stable and the environment is changeless. The models trained merely on these datasets may be adaptive to dataset-specific attributes and less generic. 

%\end{widelist}

%Though some previous works have tried to tackle this problem with a auxiliary task like expression recognition by utilizing extra dataset, their performance are still limited to the data scale because their supervised training strategy.
To address the above problems, our efforts are on constructing a powerful and robust facial representation pre-trained on a large set of face images. Since the pre-training datasets are scrabbed from web and totally in the wild, they contains numerous expressions, numerous identities and various attributes. This is conducive to relieve the distribution imbalance problems of AU class and combinations, and to reduce the overfitting to unexpected identities and environments.


% %%%%%%%%%%%%%%%%
% \subsection{Framework Overview}

% \textcolor{red}{The basic idea is to pre-train a strong and generic facial representation for the down-stream AU-related tasks with no need for labeled data.} Our proposed framework contains two modules, namely a feature extractor based on pre-trained MAE and a classifier head. As shown in Figure\ref{fig:pipeline}, our training procedure includes two stages, namely pre-training task stage (Stage~1) and AU-related task stage (Stage~2). The framework of Stage~1 relies on MAE, which contains a ViT\cite{ViT} \textcolor{red}{ViT definition, its full name} encoder and a light decoder. Stage~2 contains the same ViT encoder pre-trained from Stage~1 while it has a linear head to output the predicted AU results(occurrence probability or intensity value).

% In Stage~1, the input facial data are randomly sampled from large scale facial datasets without AU anotations. Its target is to train a strong and robust facial feature extractor. In Stage~2, we utilize the ViT encoder pre-trained in Stage~1 as our feature extractor to extract powerful facial features. Particularly, in this stage, the input facial data are randomly sampled from AU datasets and not masked, in other word, all the pathches of input data are fed into the pre-trained ViT encoder. We fine-tune the whole network and update the whole network's parameters when training with AU-related tasks.


% %%%%%%%%%%%%%%%%
% \subsection{MAE Feature Extractor Pre-training}
% \label{section:method:mae_pretrain}

% Unlike other pre-training works for facial action unit which is either directly on AU detection task or on related task like expression recognition with limited labeled data, our insight is to fully tap the potential of numerous facial data without annotation. Following MAE, we take advantage of the encoder-decoder structure as our pre-training framework. This section will introduce the details of our data processing and network pre-training.

% % MAE Pre-training
% \textbf{Pre-training with Masked Image Encoding.} \textcolor{red}{We choose a simple yet efficient pre-training task, a self-supervised paradigm that partially masks the facial image patches and then reconstructs them.} The encoder and decoder are denoted as $f(\cdot)$ and $d(\cdot)$. Given a face image $I$, we first crop it into uniform non-overlapping patches $I = \{I_i\}_{n \times n}$, where n is the number of patches in the width or height direction, then we randomly sample them by a mask ratio $mr$ to get the masked patches $I^m = \{I_i\}^{mr}_{n \times n}$. The pre-training task can be denoted as:
% \begin{equation}
% \{I_i\}_{n \times n}= d(f(\{I_i\}^m_{n \times n})),
% \end{equation}

% This ensures us to obtain our strong and transferable feature extractor $f(\cdot)$ \textcolor{red}{WHY, we have to make it clearly.}.
% A prominent option is the mask ratio $mr$. By masking out a large portion of the image
% patches ($mr=75\%$), \textcolor{red}{Can we make a few experimental comparisons to show the best portion of $mr=75\%$.} the MAE encoder is forced to extract high-level semantic information from the patches, where low-level features are not enough to predict the original image
% contents.\textcolor{red}{Can we provide a few intermediate experimental results to confirm that.}


% \textbf{Pre-training Details.}
% Following MAE\cite{MAE}, we keep most of the pre-training setups the same, except for four aspects.

% Firstly, the pre-training dataset is different. We pre-train the model with facial image datasets, designed specifically for facial analysis tasks. 

% Secondly, we use ViT-Base as the backbone in our experiments. As long as more computational resources are available, the results in this paper can be further improved with bigger backbone such as ViT-Large, ViT-Huge or ViT-Huge-448 variants. Rather than using bigger models, ViT-Base backbone shows the effectiveness of the method itself. More importantly, the ViT-Base model is more feasible for deploying.

% Thirdly, since the face dataset is a subset of the general image dataset, instead of pre-training from scratch, we initialize the encoder weights from ImageNet-1k pre-trained MAE. This will boost the pre-training stage, requiring less epochs to converge. Note that it's also viable to pre-train from scratch as in the original MAE. In our early experiments, the AU model pre-trained from scratch still outperforms the previous bests. \textcolor{red}{do we provide experimental resutls?}

% Lastly, L1 loss is used as the loss function, replacing mean squared error (aka. L2 loss) proposed in the original MAE. As MAE directly reconstructs pixels, and L1 loss usually performs better than L2 loss in image restoration problems\cite{zhao2015loss}, L1 loss is worth a try in MAE pre-training. In our experiments, L1 pre-trained MAE improves sharpness of the reconstructed images, and fine-tuned MAE also performs better with L1 pre-training.


% \textbf{Pre-training Dataset \& Pre-processing.}
% We build up our pre-training dataset from 4 datasets, designed for various facial tasks, These datasets are concatenated to form a large set. The size of the combined dataset is about 2,170,000, with all the labels removed. 
% \begin{enumlist}
% \item AffectNet\cite{AffectNet}, 960,000 images
% \item CASIA-WebFace\cite{CASIA-WebFace}, 494,000 images
% \item IMDB-WIKI\cite{IMDB-WIKI}, 514,000 images
% \item CelebA\cite{CelebA}, 203,000 images
% \end{enumlist}

% The proposed pre-training dataset is not very large. This benefits from the pre-training mechanism of MAE, where 75\% of the input image patches are masked out. The random masking can be viewed as strong data augmentation, which regularizes the training procedure and prevent overfitting even after 1600 epochs.

% Nevertheless, we can still benefit from large-scale pre-training to further improve the performance. As labels are not required, it's quite easy to scale up the pre-training dataset from any dataset with face images. e.g. LAION-Face\cite{FaRL} consists of ~50M facial image-text pairs, which are face images extracted from LAION-400M\cite{LAION-400M}.

% The pre-training data are pre-processed as following:
% \begin{enumlist}
% \item We clean up the dataset by dropping corrupt files and images with too low resolution, e.g. either width or height is less than 64 (the threshold may change for each dataset).
% \item RetinaFace\cite{RetinaFace} is applied to detect faces and 5-point facial landmarks. Images with no face detected are dropped. Face images are aligned by rotating, bilinear interpolation is applied to suppress aliasing. The rotation angle is extracted from the coordinates of the two eyes in the facial landmarks.
% \item RetinaFace is applied again to detect facial bounding box. A square region containing the bounding box is cropped to get the final face image.
% \end{enumlist}


%%%%%%%%%%%%%%%%
\subsection{Framework Overview}

We build up a two-stage framework to tackle the AU-related tasks, following the training paradigm of MAE\cite{MAE}. Our framework is pre-trained in Stage~1 to learn a robust facial representation, namely \textbf{MAE-Face}, and then fine-tuned in Stage~2 for a specific AU-related task.

\textcolor{red}{Let's talk about what benefits by Stage~1 and stage 2, or two-stage. Not involving methods e.g. super-supervised manner.}

\textcolor{red}{Stage~1 is built up with Vision Transformer (ViT)\cite{ViT}. After showing its success in NLP\cite{Transformer}, Transformer has also shown competitive performance in computer vision\cite{ViT} with regard to convolutional nerual network (CNN)\cite{CNN}. We choose the ViT-Base variant as our backbone because it's a relatively small and fast variant of ViT, which is also suitable for deployment.}

%%%%%%%%%%%%%%%%
\subsection{Facial representation pre-training}
\label{section:method:mae_pretrain}

In Stage~1, a facial representation model is learned by pre-training on face images.
The model is pre-trained in a self-supervised manner, which means there's no need for labeled data and only face images is required for learning. In this way, we can easily utilize a large set of in-the-wild face images for pre-training.

Among the various self-supervised vision learning methods, we utilize masked autoencoding as our pre-training paradigm to obtain a high-capacity model as the backbone for AU detection and AU intensity estimation.
The pre-trained model is an autoencoder built up by a ViT-Base encoder and a ViT decoder, where the encoder has a depth of 12 and a width of 768, and the decoder has a depth of 8 and a width of 512.

\textbf{Masking}.
We follow a masking-and-reconstruct procedure for the pre-training. Before feeding into the model, an image is uniformly splitted into non-overlapping patches of $16\times16$. Positional embedding\cite{Transformer} is used to mark the relative position of the patches. We mask out 75\% of the image patches and only 25\% patches are used as the input for pre-training. With this masking operation, the model only has a partial observation of the input image, where a lot of the original information is missing. The training target for the ViT autoencoder is to reconstruct the original image, which means the model tries to predict the missing patches as close as possible.

\textbf{Loss function}.
We use L1 loss as the reconstruction loss. Unlike the original MAE\cite{MAE} which uses L2 loss, we find that the model pre-trained with L1 loss exhibits better performance in downstream tasks (please refer to Section~\ref{section:ablation:pretrain_loss_function}). This conclusion is consistent with a prior work about the loss functions in image processing\cite{zhao2015loss}, where L1 loss show superiority over L2 loss in most cases.

\textbf{Initialization}.
Instead of random initialization, we initialize the ViT encoder using the ImageNet-1k pre-trained encoder released by \cite{MAE}. This will speed up the pre-training procedure, where a 200-epoch pre-trained model can exhibit decent performance in downstream tasks (e.g. in Section~\ref{section:ablation:pretrain_loss_function}). Nevertheless, we can still benefit from a longer pre-training, so we use 800 epochs in most of our experiments.

\textbf{Dataset}.
We build up our pre-training dataset from 4 datasets, designed for various facial tasks:
\begin{enumlist}
\item AffectNet\cite{AffectNet}, 960,000 images;
\item CASIA-WebFace\cite{CASIA-WebFace}, 494,000 images;
\item IMDB-WIKI\cite{IMDB-WIKI}, 514,000 images;
\item CelebA\cite{CelebA}, 203,000 images.
\end{enumlist}
These datasets are concatenated to form a large set. The size of the combined dataset is about 2,170,000, with all the labels removed.
The proposed pre-training dataset is not very large. This benefits from the pre-training mechanism of masked autoencoding.
The high-ratio random masking can be viewed as a strong data augmentation, which regularizes the training procedure and prevent overfitting even after 1600 epochs.
Nevertheless, we can still benefit from large-scale datasets to further improve the performance.

\textbf{Pre-processing}.
The pre-training data are pre-processed as following:
\begin{enumlist}
\item We clean up the dataset by dropping corrupt files and images with too low resolution, e.g. either width or height is less than 64 (the threshold may change for each dataset).
\item RetinaFace\cite{RetinaFace} is applied to detect faces and 5-point facial landmarks. Images with no face detected are dropped. Face images are aligned by rotating, bilinear interpolation is applied to suppress aliasing. The rotation angle is extracted from the coordinates of the two eyes in the facial landmarks.
\item RetinaFace is applied again to detect facial bounding box. A square region containing the bounding box is cropped to get the final face image.
\end{enumlist}


% %%%%%%%%%%%%%%%%
% %\subsection{Transfer Learning on Action Units.}
% \subsection{End-to-end fine-tuning on Action Units}

% The pre-training task yields a powerful feature extractor, which can capture fine-grained facial features, served as an optimal network initialization. Thus in downstream tasks, we can train our AU detection network and AU intensity estimation network with limited labeled data. This section will introduce the implementation details for fine-tuning.

% \textbf{Fine-tuning on Action Unit.}
% In fine-tuning stage, all image patches are fed into the MAE encoder without masking. We extract features from the encoder output. The MAE decoder is dropped because there's no more need for reconstructing pixels. Then, global average pooling is applied to the features, followed by a LayerNorm\cite{LayerNorm}. Finally, a fully connected layer is added to the end of the network, served as the classification head.

% \textbf{Pre-processing for fine-tuning Datasets}: same as (2) and (3) in pre-training pre-processing, face detection, face alignment and face cropping is applied to extract aligned face images from the original datasets.

% In common practices, face detection and face alignment plays an important role in facial recognition tasks. Therefore, it's naturally to perform face alignment before feeding a face image to the AU model. We follow this practice in our fine-tuning stage, but a question raises in the pre-training stage.

% By reconstructing pixels from natural images, the original MAE yields a generic image encoder, which can be easily adapted to various downstream vision tasks. What about MAE-Face? With aligned face images for both pre-training and fine-tuning, it is expected to be good in experimental cases, but may at the price of losing generality, e.g. lower precision when predicting non-aligned faces. With detailed experiments, We will explain this question in Section~\ref{section:ablation:data_preprocessing}.


%%%%%%%%%%%%%%%%
\subsection{End-to-end fine-tuning on Action Units}

In Stage~2, the pre-trained model is fine-tuned on AU datasets for AU detection or AU intensity estimation.
Following \cite{MAE}, we apply an end-to-end fine-tuning mechanism instead of linear probing to obtain the highest performance.

We drop the pre-trained ViT \textbf{decoder} because it is designed for use in reconstructing pixels but not in downstream tasks.
However, after learning a robust facial representation, the pre-trained ViT \textbf{encoder} serves as the key component in our framework.

\textbf{Classifier}.
We build up our classifier using the pre-trained ViT encoder followed by a global average pooling, a Layer Normalization\cite{LayerNorm} and a fully-connected layer as the classification head.
The encoder is supposed to learn a facial expression representation and the head is supposed to learn a linear mapping to the final output.

\textbf{Fine-tuning on AU datasets}.
During fine-tuning, all image patches are fed into the model without masking, and the optimization target is to detect AU occurance or to estimate AU intensity.
We optimize both the encoder and the head using back propagation.
Finally, the optimization iteration stops when the validation loss has stopped decreasing.

\textbf{Pre-processing}.
Same as the pre-processing in pre-training, face detection, face alignment and face cropping is applied to extract aligned face images from the original AU datasets.
In common practices, face detection and face alignment plays an important role in facial recognition tasks. Therefore, it's naturally to perform face alignment before feeding a face image to the AU model. We follow this practice in our fine-tuning stage, but a question raises in the pre-training stage.


%%%%%%%%%%%%%%%%
\subsection{Loss Functions}
% AU Detection Fintuning
% AU Intensity Estimation Fintuning

Our pre-training procedure is a mask-then-predict task, which aims to predict the masked patches. The loss of pre-training task is $\mathcal{L}_{pre}$. We then validate our pre-trained model on both AU detection and AU intensity estimation tasks, whose losses are denoted as $\mathcal{L}_{det}$ and $\mathcal{L}_{int}$, respectively, each of them is introduced in detail in the following.

\textbf{Loss of MAE pre-training.} Suppose there are $K$ masked patches in the input $I^m = \{I_i\}^{mr}_{n \times n}$. To predict the $K$ masked patches accurately, we utilize pixel-wise L1 loss to constrain the distance between the prediction ($\hat m_k$) and ground-truth ($m_k$) of the masked patches. Thus ${L}_{pre}$ can be denoted as:
\begin{equation}
\mathcal L_{pre} = \sum_{k=1}^{K} || m_k - \hat m_k ||,
\end{equation}

\textbf{Loss of AU detection.} To constrain the AU detection results to be as close as possible with AU ground-truth, we formulate it as a multi-label binary classification problem, where each AU label is a binary. Thus $\mathcal{L}_{det}$ is defined as:
\begin{equation}
\mathcal L_{det} = -\sum_{i=1}^{N} [p_i log \hat{p}_i + (1 - p_i) log(1-\hat{p}_i)],
\end{equation}
where $N$ is the number of AUs, $\hat p_i$ denotes the predicted probability which is the model output activated by a sigmoid function, and $p_i$ denotes the binary ground-truth of $AU_{i}$.

\textbf{Loss of AU intensity estimation.} Since the AU intensity values are annotated as discrete integers in 0$\sim$5, we normalize the ground-truth values to 0$\sim$1. Then, the goal of our model is to regress the normalized AU intensity values. We use L2 distance to minimize the distance between the predicted value $\hat v_i$ and ground-truth $v_i$ for $AU_{i}$, thus $\mathcal{L}_{int}$ is denoted as:
\begin{equation}
\mathcal L_{int} = \sum_{i=1}^{N} || v_i - \hat v_i ||^2_2,
\end{equation}
During inference, the model output is scaled to the original 0$\sim$5 range for evaluation.


==> zzz.backup/method_mbw.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Method}
\label{section:method}


To train an AU model, training from scratch can be quite difficult. Since AU datasets require manually annotated labels by experts, the sizes of nearly all the AU datasets are limited. When training from scratch, the model tends to overfit and easily converges to a bad local minima, implying that the major challenge in training an AU model is about better optimization. Traditional methods require prior knowledge about AU and task-specific designs. While from the perspective of modern deep learning, pre-training turns out to be the solution.

Since AUs describe facial expressions, it's straightforward to supervisely pre-train from a facial expression dataset other than AU's. As far as we know, AffectNet[] is the largest facial expression dataset openly available, which contains 420k manually annotated images. In spite of the fact that it's still not a very large-scale dataset, with noisy annotations and the imbalanced classes, training AffectNet itself will be another challenging task.

Therefore, we turn to self-supervised pre-training.

%%%%%%%%%%%%%%%%
\subsection{Pre-training with Masked Image Encoding}

\textbf{Masked autoencoder (MAE)}[] introduced a self-supervised method to pre-train from image dataset without labels or extra tokens.

In pre-training stage, MAE is built up by an encoder and a decoder. Both the encoder and decoder are Vision Transformers (ViT)[]. The ViT encoder accepts a stack of image patches as the input, where 75\% of the patches are masked out. Then, the encoded patches and mask tokens are fed into the ViT decoder to reconstruct the original image in pixels. This procedure is called \textbf{masked image encoding}.

In natural language processing (NLP), BERT[] and GPT[] show great success in self-supervised pre-training, enabling scaling up the model size and data size to a very large scale. As a pioneer in masked autoencoding, BERT uses a mask ratio of 15\%, much lower than 75\% in MAE. This is because there's much more redundancy and spatial correlation in natural image pixels than in natural language words. For example, we can easily down-sampling an image to 1/16 pixels and still recognize most of the image contents, with losses only in details and textures. However, if we drop 15/16 words in an article, it will be hard to tell what it is talking about.

A similar task, image inpainting, usually predicts missing image pixels from low-level image features such as textures and shapes. One of the key difference in MAE is the mask ratio. By masking out a large portion of the image patches (75\%), the MAE encoder is forced to extract high-level semantic information from the patches, where low-level features are not enough to predict the original image contents.

As an alternative masked image encoding method, BEiT[] predicts tokens instead of reconstructing pixels. BEiT introduces an extra pre-trained dVAE[Zero-shot text-to-image generation] as the tokenizer, which requires extra data for the pre-training, the use of tokenizer also slows down the pre-training stage in masked image encoding. Thus, we choose MAE as it's simpler to implement and faster to train.

%%%%%%%%%%%%%%%%
\subsection{Pre-training Details}

Following MAE[], we keep most of the pre-training setups the same, except:
\begin{enumlist}
\item We pre-train the model with facial image datasets, designed specifically for facial analysis tasks.
\item We use ViT-Base as the backbone in our experiments. As long as more computational resources are available, the results in this paper can be further improved with bigger backbone such as ViT-Large, ViT-Huge or ViT-Huge-448 variants. Rather than using bigger models, ViT-Base backbone shows the effectiveness of the method itself. More importantly, the ViT-Base model is more feasible for deploying.
\item Since the face dataset is a subset of the general image dataset, instead of pre-training from scratch, we initialize the encoder weights from ImageNet-1k pre-trained MAE. This will boost the pre-training stage, requiring less epochs to converge. Note that it's also viable to pre-train from scratch as in the original MAE. In our early experiments, the AU model pre-trained from scratch still outperforms the previous bests.
\item L1 loss is used as the loss function, replacing mean squared error (aka. L2 loss) proposed in the original MAE. As MAE directly reconstructs pixels, and L1 loss usually performs better than L2 loss in image restoration problems[], L1 loss is worth a try in MAE pre-training. In our experiments, L1 pre-trained MAE improves sharpness of the reconstructed images, and fine-tuned MAE also performs better with L1 pre-training.
\end{enumlist}

%%%%%%%%%%%%%%%%
\subsection{Pre-training Datasets}

We pre-train MAE with 4 datasets, designed for various facial tasks:
\begin{inlinelist}
\item AffectNet[]: ~960k, unaligned
\item CASIA-WebFace[]: ~494k, unaligned
\item IMDB-WIKI[]: ~514k, unaligned
\item CelebA[]: ~203k, aligned
\end{inlinelist}

These datasets are concatenated to form a large set. The size of the combined dataset is ~2.17M, with all the labels removed.

The proposed pre-training dataset is not very large. This benefits from the pre-training mechanism of MAE, where 75\% of the input image patches are masked out. The random masking can be viewed as strong data augmentation, which regularizes the training procedure and prevent overfitting even after 1600 epochs. This also explains why MAE can achieve the best result in image classification when pre-trained with ImageNet-1k only.

Nevertheless, we can still benefit from large-scale pre-training to further improve the performance. As labels are not required, it's quite easy to scale up the pre-training dataset from any dataset with face images. e.g. FaRL[] proposed to build up LAION-Face dataset by extracting face images from LAION-400M dataset[], which consists of ~50M facial image-text pairs.

%%%%%%%%%%%%%%%%
\subsection{Fine-tuning on Action Unit}

In fine-tuning stage, all image patches are fed into the MAE encoder without masking. We extract features from the encoder output. The MAE decoder is dropped because there's no more need for reconstructing pixels. Then, global average pooling is applied to the features, followed by a LayerNorm[]. Finally, a fully connected layer is added to the end of the network, served as the classification head.

%%%%%%%%%%%%%%%%
\subsection{Data Pre-processing}
\label{section:methods:data_preprocessing}

\textbf{For pre-training datasets:}
\begin{enumlist}
\item We clean up the dataset by dropping corrupt files and images with too low resolution, e.g. either width or height is less than 64 (the threshold may change for each dataset).
\item RetinaFace[] is applied to detect faces and 5-point facial landmarks. Images with no face detected are dropped. Face images are aligned by rotating, bilinear interpolation is applied to suppress aliasing. The rotation angle is extracted from the coordinates of two eyes from the facial landmarks.
\item RetinaFace is applied again to detect facial bounding box. A square image is cropped based on the bounding box.
\end{enumlist}

\textbf{For fine-tuning datasets:} same as (ii) and (iii) in pre-training, face detection, face alignment and face cropping is applied to extract aligned face images from the original datasets.

In common practices, face detection and face alignment plays an important role in facial recognition tasks. Therefore, it's natually to perform face alignment before feeding a face image to the AU model. We follow this practice in our fine-tuning stage, but a question raises in the pre-training stage.

By reconstructing pixels from natural images, the original MAE yields a generic image encoder, which can be easily adapted to various downstream vision tasks. What about MAE-Face? With aligned face images for both pre-training and fine-tuning, it is expected to be good in experimental cases, but may at the price of losing generality, e.g. lower precision when predicting non-aligned faces. With detailed experiments, We will explain this question in Section~\ref{section:ablation:data_preprocessing}.

==> zzz.backup/related_work_bak_20221010.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Related Works}
Lots of works on AU detection and intensity estimation have been proposed in recent years. This section will represent the previous woks about their contributions and deficiencies. Finally, we represent some advance self-supervised learning works highly related to our frameworks.
%%%%%%%%%%%%%%%%
\subsection{AU Detection}
Conventional AU detection works often utilize hand-craft features like Gabor wavelet features\cite{valstar2006fully}, LBP\cite{jiang2011action,LP48}, SIFT\cite{zeng2015confidence} to detect AU by classfiers with Adaboost or SVM, etc. Recently deep learning based methods boost the performance of AU detection to a new level. Considering the local region of AU, many previous works\cite{Onal2019D-PAttNet}\cite{JPML} detect AU based on patch learning. For instacne, Zhao \textit{et al} \cite{DRML} divide facial images uniformly into several parts, and extract feature individually to detect AU. Joint patch and multi-label learning are proposed in\cite{JPML} to recognize AU, in which the landmark detection are introduced to select important facial patches. Ma \textit{et al}\cite{ma2019r} define an AU partition rule based on expert prior knowledge and ultilize R-CNN based model to recognize AU in different ROI. More recently, Ge \textit{et al} \cite{ge2021local} propose a muti-branch network to exploit the relationship among multiple patches, not only exploiting the correspondence of different AUs but also considering other non-AU regions. They further introduce multi-level graph attention to enhance AU features learning\cite{ge2022mgrr} and get performance improvement. These works make effort to efficiently extract facial features but neglect the data scarcity thus limited by the lack of data.

Due to the correlation existing in AUs, the AU relationship modeling has also been explored by lots of works to improve recognition accuracy. Tong \textit{et al} \cite{tong2007facial} utilize dynamic Bayesian network to model the relation of various AUs. Niu \textit{et al}\cite{LP} obtain local features and learn the relationships in different local regions via relationship learning. Corneanu \textit{et al}\cite{corneanu2018deep} use a deep model to extract local and global features, then capture structure between patches with a message passing algorithm. Liu \textit{et al}\cite{liu2020relation} capture AU local features via auto-encoder and then learning AU relationships with a GCN model. Li \textit{et al}\cite{SRERL} propose a semantic relationship embedded representation learning network(SRERL) with a structured knowledge-graph to organize the facial AUs and enhance AU representation learning. These works demonstrate the effectiveness of AU relation modeling. However, the data scarcity still restricts their performance.

With the success of attention mechanism, it has also been deployed in AU detection. Li \textit{et al} propose an attention based method, EAC-Net\cite{EAC-Net}, which conducts attention learning with rough facial landmarks. Attention is predefined by prior AU center. Ertugrul \textit{et al}\cite{Onal2019D-PAttNet} deploy sigmoid attention on patch features which are encoded individually. Shao \textit{et al}\cite{shao2021jaa} treat face alignment and AU detection as a joint task, proposing an adaptive attention learning module to refine each AU attention map. They further utilize channel and spatial wise attention to adaptively learn AU-related local features\cite{attnetionTrans2019}. Recently Jacob \textit{et al}\cite{jacob2021facial} encode image feature via transformer encoder and learn attention map for each AU via a ROI attention module, focusing on AU-related spatial regions. Attention mechanism has been demonstrated to be effective for AU recognition in these works, whereas they are merely trained on limited data which leads to poor generalization.

To break through the limitation of data scarcity, some recent works consider to introduce extra data or auxiliary information to aid AU detection. For instance, Cui \textit{et al}\cite{cui2020knowledge} combine facial expression recognition with action unit detection, and train them jointly to refine their learning. Yang \textit{et al} \cite{yang2021exploiting} using textual descriptions of AUs occurrence to capture different AU semantic relations, exploiting semantic embedding and visual feature for AU detection. Zhao \textit{et al}\cite{zhao2018learning} utilize large-scale web images with inaccurate annotations to faciliate AU detection. Chen \textit{et al}\cite{chen2022causal} focus on removing the effect caused by subject variation in AU recognition via a causal intervention module. More recently, to alleviate the reliance on densely annotated data, Li \textit{et al}\cite{li2022knowledge} propose to learn the interactive spatial-temporal correlation with extremely limited annotated data, consistency regularization and pseudo-labeling to make the learning progress more efficient.
\subsection{AU Intensity}
Probabilistic models\cite{rudovic2012multi,rudovic2012kernel,eleftheriadis2017gaussian} are extensively explored in AU intensity estimation. For instance, Walecki \textit{et al} \cite{walecki2017deep} model AU co-occurrence patterns of AU intensity levels by comnining conditional random field(CRF). Eleftheriadis \textit{et al} \cite{eleftheriadis2016variational} propose Gaussian process auto-encoder for AU intensity estimation, which projects features via a encoder onto a latent space and reconstruct them to original features via a decoder. Markov Random Fields\cite{sandbach2013markov} and Conditional Ordinal Random Fields\cite{rudovic2012kernel}\cite{rudovic2012multi} are also been applied for predicting AU intensity.

Works\cite{zhang2018weakly}\cite{zhang2018bilateral}\cite{zhang2019joint} leveraging deep models to solve AU intensity estimation problem also emerge in recent years. Zhang\textit{et al}\cite{zhang2019joint} propose a novel weakly supervision training method with human knowledge to learn representation and intensity simultaneously. They also exploit another weakly supervised method that learns frame-level intensity estimator and makes use of weakly labeled sequences data\cite{zhang2018bilateral}. Sánchez-Lozano \textit{et al}\cite{HR} jointly perform AU localisation and intensity estimation through heatmap regression. Fan \textit{et al}\cite{SCC-Heatmap} design a heatmap regression-based model and encode visual patterns of AUs in feature channels, reflecting the AU co-occurring pattern by the feature channels activation set.

More recently, context-aware temporal feature fusion and label fusion are applied in estimating AU intensity\cite{zhang2019context}\cite{sanchez2021affective}. Zhang \textit{et al}\cite{zhang2019context} considering utilizing part of annotated databases and propose a weakly supervised patch-based framework for regressing AU intensity. They design a context-aware feature fusion module to capture spatial relationships among various local patches, and a context-aware label fusion module to capture the temporal dynamics. Sanchez \textit{et al}\cite{sanchez2021affective} present a novel way to model temporal context based on neural processes, which contains global stochastic contextual representation, task-aware temporal context modeling and selection.


%%%%%%%%%%%%%%%%
\subsection{AU Tasks with Auxiliary Information}
The AU annotation process requires very professional knowledge and even to experts, it takes much time and effort to label a video. As a result, the commonly used AU datasets~(e.g., BP4D\cite{BP4D}, DISFA\cite{MavadatiDISFA}) contain limited identities and data, which may lead to overfitting to the trainset.
To relieve, several works propose to introduce the auxiliary information to enhance the generalization. 
The facial landmarks contain the facial geometry information, which is often used in AU-related tasks. 
LP-Net\cite{LP} applies the landmarks to extract the shape feature. 
J{\^A}A-Net\cite{shao2021jaa} proposes a multi-task framework that combines landmark detection and AU detection. 
Likely, Jacob et al.\cite{jacob2021facial} perform a multi-tasks of AU detection and landmark-based attention map prediction.
However, the performance of these methods limits to the effectiveness of landmarks detection. Also, the landmarks also introduce the identity information, which may damage the generalization. 

Textual information can be also used in AU tasks. SEV-Net\cite{yang2021exploiting} utilizes the extra annotation of descriptions of AUs and introduces the pre-trained word embedding model to facilitate generating the AU-related attention map. However, the textual annotation also requires much effort and time.


Zhang et al.\cite{zhang2021prior} introduce the pre-trained expression embedding\cite{zhang2021learning} feature as prior knowledge to enhance the AU detection. The expression embedding space is compact, which can represent the fine-grained human expressions without disturbance of identities, poses and illumination. But the limited faces used in the pre-trained prior model still restrain the performance of AU tasks.


%%%%%%%%%%%%%pipeline figure
\begin{figure*}[!t]
    \centering
    \includegraphics[ width=18cm]{images/MAE_pipeline_4.pdf}
    %\vspace{-0.5em}
    \caption{The schematic pipeline of the proposed global-to-local expression-aware embeddings AU detection framework. It is composed of three main modules: the Global Expression representation Encoder(\textsl{GEE}), local AU features module(\textsl{LAM}), and AU classifier. The \textsl{GEE}, pre-trained by expression similarity tasks with the triplet loss, extracts a global expression feature map from the input image, which is capable of sensing subtle expression changes. The global expression feature is then fed into the AU Mask Extractor($E_m$) and the AU Feature Map Extractor($E_a$). The two extractors produce AU-specific masks and feature maps from the global expression feature($h$), respectively. AU masked features are obtained through pixel-wise product on the outputs of two extractors, which are then fed into the following AU Classifier to obtain the AU embeddings and detection results.}
    \label{fig:pipeline}
\end{figure*}
%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%
\subsection{Self-supervised Learning}

Recent years, \textbf{masked language modeling} has shown great successes in NLP. Auto-encoding models, such as BERT\cite{BERT}, are pre-trained to reconstruct missing contents corrupted by random masking. Auto-regressive models, such as GPT\cite{GPT}, are pre-trained to predict next token based on all the previous ones. With no need for labeled data, masked \textcolor{red}{language modeling can easily increase the dataset size} as well as the model size to a very large scale, improving the performance for downstream tasks by a lot.

Meanwhile, self-supervised vision representation learning is also a research hotspot. Contrastive learning\cite{wu2018unsupervised}\cite{oord2018representation}\cite{hjelm2018learning}\cite{bachman2019learning}\cite{he2020momentum}\cite{chen2020simple} is a popular one of them. \textcolor{red}{It proposes to learn from the images with carefully designed augmentations, where the model tries to represent the positive pairs as close as possible and the nagative pairs as far as possible.} In this way, the model is forced to extract high-level semantic features, ignoring low-level pixel-wise features which are easily influenced by the augmentations.

\textbf{Masked image modeling}, as a straightforward idea similar to masked language modeling, has been tried but not shown many successes\cite{ViT}. Until recently, BEiT\cite{BEiT} comes up with a pre-training framework to predict visual tokens of the missing patches with masked image patches as the input. As an alternative, MAE\cite{MAE} proposes to directly reconstruct pixels of the masked patches. The general intuitions of BEiT and MAE are the same. BEiT follows common NLP routines using tokens, while MAE is a more straightforward method natively designed for image modeling.

BEiT uses a pre-trained discrete VAE from DALLE\cite{DALLE} to generate predicted tokens, where the dVAE is pre-trained with extra data (250M images). Since we want to build a vision representation for face images specifically, the dVAE trained with general images\cite{DALLE} may not be the optimal tokenizer for our problem. Besides, in BEiT pre-training, the dVAE inference also brings extra computation. With no need for a tokenizer, MAE is much simpler to implement and also faster to train. Thus, we build our pre-training framework based on MAE as the self-supervised vision representation learner.

